Joins on Samples: A Theoretical Guide for Practitioners

Despite decades of research on approximate query processing (AQP), our understanding of sample-based joins has remained limited and, to some extent, even superficial. The common belief in the community is that joining random samples is futile. This belief is largely based on an early result showing that the join of two uniform samples is not an independent sample of the original join, and that it leads to quadratically fewer output tuples. However, unfortunately, this result has little applicability to the key questions practitioners face. For example, the success metric is often the final approximation's accuracy, rather than output cardinality. Moreover, there are many non-uniform sampling strategies that one can employ. Is sampling for joins still futile in all of these settings? If not, what is the best sampling strategy in each case? To the best of our knowledge, there is no formal study answering these questions. This paper aims to improve our understanding of sample-based joins and offer a guideline for practitioners building and using real-world AQP systems. We study limitations of offline samples in approximating join queries: given an offline sampling budget, how well can one approximate the join of two tables? We answer this question for two success metrics: output size and estimator variance. We show that maximizing output size is easy, while there is an information-theoretical lower bound on the lowest variance achievable by any sampling strategy. We then define a hybrid sampling scheme that captures all combinations of stratified, universe, and Bernoulli sampling, and show that this scheme with our optimal parameters achieves the theoretical lower bound within a constant factor. Since computing these optimal parameters requires shuffling statistics across the network, we also propose a decentralized variant where each node acts autonomously using minimal statistics.

==> filters.tex <==
%!TEX root = main.tex

\section{Filters}
\label{sec:where}

In the presence of filters (\ie, \WHERE clause), the variance of our estimator now depends on the distributional information for join columns \emph{after} applying the filters.
Estimator can be defined similarly as before:
for \COUNT and \SUM, we compute aggregate on the UBS sample and then scale the answer by the factor $1/\pmin q_1q_2$.
To measure the quality of the estimator and the sampling scheme, there are usually two options.
When there are no distributional assumption on the parameters of the \WHERE clauses, we should consider the \emph{worst case} variance among all possible \WHERE clauses. However, from the formula~\ref{eqn:count} and formula~\ref{eqn:var-sum}, it is not hard to see that for all the sampling parameter $p$,
the variance increases as the frequencies of tables increase monotonically.
Therefore, among all possible filters, the one that gives the highest variance for our estimator must be the one that keeps all the tuples in the table with the \WHERE clause.
In other words, if our goal is to minimize the \emph{worst case} variance, we can use the optimal parameter for the query \emph{without} the \WHERE clause.
The worst case variance is thus given by Theorem~\ref{thm:opt-rate} and Theorem~\ref{thm:opt-rate-sum}.

However, since most of the \WHERE clauses are not going to leave all tuples selected,
using a parameter that is optimal only for the worst case might lead to a worse performance on average.
In the following section, we investigate the \emph{average variance} based on some distributional assumptions.
In particular, we consider the following query on join size, where we know the filter column:
\begin{verbatim}
    select count(*)
    from T1 join T2 on J
    where T1.C >= X
\end{verbatim}
The performance of our estimator depends on both the joint distribution of columns $C$ and $J$, as well as the distribution on $X$.
Here we analyze the average variance of our estimator with \WHERE clauses by taking the average over the distribution of $x$.
Note that as usual, the estimator is obtained by running the query on the sample and then scaling up its answer by a factor of $\frac{1}{\pmin q_1 q_2}$.

We consider two possible distribution of $x$:
The uniform distribution, or the same distribution as the column $C$.
Specifically, we define $m_C$ to be the number of distinct values present in column $C$, and $a_{u, v}$ be the number of tuples in $T_1$ with value $u$ in column $J$ and $v$ in column $C$.
Now we provide the average variance of our estimator for such queries in the subsequent sections.

% \subsection{WHERE clause Centralized Setting}

\subsection{WHERE Clause in Uniform Distribution}
\label{sec:where:uniform}

In this section, we first study the case where $x$ is from a uniform distribution.
The estimator is defined for the join size in Section \ref{sec:count}.
% For join size estimation, we take the join of the sample and 

In uniform distribution, $X$ takes on each value in column $C$ with equal probability, i.e. probability $1/m_C$.
For a given value $x$ of $X$,
the average variance of our estimator is given by\footnote{Further derivations and details are omitted to conserve space. Interested readers can refer to our technical report~\cite{anon_report}.}:
% \barzan{I am dubious coz you haven't even defined the estimator=} is given by:
% \begin{align*} 
%      &\var[\Jcount] \\
%     =& (\frac{1}{p} - 1) \sum_v a_{v,\geq x}^2 b_v^2 + (\frac{1}{\epsilon_2} - \frac{1}{p})\sum_v a_{v, \geq x}^2 b_v \\ 
%     & (\frac{1}{\epsilon_1} - \frac{1}{p})\sum_v a_{v, \geq x} b_v^2 + (\frac{p}{\epsilon_1 \epsilon_2} - \frac{1}{\epsilon_1} - \frac{1}{\epsilon_2} - \frac{1}{p})\sum_v a_{v,\geq x} b_v \label{eqn:var-where}
% \end{align*}
% where $a_{v, \geq x} = \sum_{u \geq x} a_{v, u}$.
% Therefore, the average variance is:
\begin{align*}
     &\overline{\var[\Jcount]} \\ 
    =& \frac{1}{m_C}\sum_x ( (\frac{1}{p} - 1) \sum_v a_{v,\geq x}^2 b_v^2 + (\frac{1}{\epsilon_2} - \frac{1}{p})\sum_v a_{v, \geq x}^2 b_v \\ 
    & (\frac{1}{\epsilon_1} - \frac{1}{p})\sum_v a_{v, \geq x} b_v^2 + (\frac{p}{\epsilon_1 \epsilon_2} - \frac{1}{\epsilon_1} - \frac{1}{\epsilon_2} - \frac{1}{p})\sum_v a_{v,\geq x} b_v )
\end{align*}

Similar to Theorem~\ref{thm:opt-rate}, the following value of $p$ will minimize the average variance in this case:
\begin{equation}
\begin{aligned}
    p = &\min\{1, \max\{\epsilon_1, \epsilon_2, \\ &\sqrt{\frac{\epsilon_1\epsilon_2\sum_{v, x} (a_{v, \geq x}^2 b_v^2 - a_{v, \geq x}^2b_v - a_{v, \geq x}b_v^2 + a_{v, \geq x}b_v)}{\sum_{v,x}a_{v, \geq x}b_v}}\}\}
\end{aligned}
 \label{eqn:where}
\end{equation}

\subsubsection{Join Size Estimation with K predicates} 
\hfill\\
Now we consider the query:

\begin{verbatim}
    select count(*)
    from T1 join T2 to J
    where T1.C1 >= x1 and T1.C2 >= x2 .... T1.Ck >= xk
\end{verbatim}

To generalize this to \WHERE clauses with $k$ columns, say $C_1, C_2, \ldots, C_k$, we define $a_{v, x_1, x_2, \ldots, x_k}$ and $a_{v, \geq x_1, \geq x_2, \ldots, \ldots, \geq x_k}$ as the number of tuples in $T_1$ that have  $C_1 = x_1, C_2 = x_2 \ldots, C_k = x_k$ and $C_1 \geq x_1, C_2 \geq x_2 \ldots, C_k \geq x_k$ respectively. Then the optimal $p$ is given by replacing $a_{v, \geq x}$ by $a_{v, \geq x_1, \geq x_2, \ldots, \ldots, \geq x_k}$ in equation~\ref{eqn:where}. 
% \textbf{Generalizing to equality filters}
\subsubsection{Join Size Estimation with K equality predicates} 
\hfill\\
We can also generalize the above result to where the filter condition is equality:
% Query:
% \begin{verbatim}
%     select count(*)
%     from T1 join T2 to J
%     where T1.C = u
% \end{verbatim}

% \subsubsection{Generalizing to K columns with equality filters}
\begin{verbatim}
    select count(*)
    from T1 join T2 to J
    where T1.C1 = x1 and T1.C2 = x2 .... T1.Ck = xk
\end{verbatim}

For the above query, the average variance minimizer is given by:
\begin{align*}
    p = &\min\{1, \max\{\epsilon_1, \epsilon_2, \\
    &\sqrt{\frac{\epsilon_1\epsilon_2\sum_{v, x} (a_{v, x}^2 b_v^2 - a_{v, x}^2b_v - a_{v, x}b_v^2 + a_{v, x}b_v)}{\sum_{v,x}a_{v, x}b_v}}\}\}.
\end{align*}
And similarly to multi-column equalities, which we will leave to readers.

% \barzan{the above equation is the most important result of this paper, so we need to fully understand and explain it:
% \begin{enumerate}
% \item how useful is this formula? i.e., is computing this more efficient than computing the join (in terms of time and space complexity)?
% Answer: Calculating $a_{v, \geq u}$ for all $v$ ``is basically'' applying the filter to the table $T_1$. And to calculate the summation, you are required to go over a  ll possible join values. Some terms, such as the one on the denominator, is just exactly the value of the query. 

% Correct Answer: Practical. (1) Can reuse sample. (2) Memory footprint for calculating the formula is much smaller than the join. Time complexity:  Memory complexity: 
% ``

% \item \textbf{the most interesting question: how to compute optimal p as efficiently as possible} how well can we estimate this quantity using a sample of T1 or T2 or both?

% \item \textbf{interesting question} how well can we estimate this quantity using a sketch of T1 or T2 or both?

% \item does our prev result still apply in saying that the other party should also follow the same p? if yes, point this out.

% \end{enumerate}
% }

% \paragraph{Identical Distribution}
\subsection{WHERE Clause in Identical Distribution}
\label{sec:where:identical}

Now we investigate when $X$ follows the same distribution as that of the column. More specifically, consider the query:
\begin{verbatim}
    select count(*)
    from T1 join T2 to J
    where T1.C = X
\end{verbatim}

Let $c_x$ be the number of tuples with value $x$ on column $C$, then the probability of $C = x$ is equal to $c_x / n_1$. % dy: |T_1| was previously n_2 <-- what is this?
We can then formulate the average case variance of the estimator as follows:

\begin{align*}
    &\overline{\var[\Jcount]} \\
   =& \frac{1}{n_1}\sum_x ( (\frac{1}{p} - 1) c_x \sum_v a_{v,x}^2 b_v^2 + (\frac{1}{\epsilon_2} - \frac{1}{p}) c_x\sum_v a_{v, x}^2 b_v \\ 
   =& (\frac{1}{\epsilon_1} - \frac{1}{p}) c_x\sum_v a_{v, x} b_v^2 + (\frac{p}{\epsilon_1 \epsilon_2} - \frac{1}{\epsilon_1} - \frac{1}{\epsilon_2} - \frac{1}{p})c_x\sum_v a_{v,x} b_v )
\end{align*}

Then the parameter $p$ that minimize this quantity is 
\begin{align*}
    p =& \min\{1. \max\{\epsilon_1, \epsilon_2, \\ &\sqrt{\frac{\epsilon_1\epsilon_2\sum_{x} c_x \sum_v (a_{v, x}^2 b_v^2 - a_{v, x}^2b_v - a_{v, x}b_v^2 + a_{v, x}b_v)}{\sum_{v,x} c_x a_{v, x}b_v}}\}\}
\end{align*}
% \barzan{Dawei, plz add this} \dawei{fixed}

% \textbf{\Large Distributed Setting}



% \section{Other Join-related Results}

% \section{Action Plan}

% \begin{enumerate}

 
 
% \item What happens if we have a where clause? Can we still guarantee anything? Under what assumptions or knowledge of the the columns in the where clause we can still hope for an optimal sampling strategy

% \begin{enumerate}
%     \item what if we don't know which columns are going to appear in the WHERE clause? Give a negative result about the best thing we can guarantee
    
%     \item When we know which columns appear in the WHERE clause but don't know which constants will be used for them? e.g., WHERE A > a and B > b where A and B are column names but the value of a and b are unknown to us at the time of sampling
    
%     \item  What if we know that the where clause will have a  subset of $\{A_1>a_1, \cdots, A_k>a_k \}$ where $A_i$ is a column name but $a_i$ is an unknown value.

%     \item  What if we know that the where clause will have a  subset of $\{A_1>a_1, \cdots, A_k>a_k \}$ where $A_i$ is a column name that appears in the WHERE clause with probabilility $p_i$ but $a_i$ is an unknown value.
%     $\{p_1,\cdots,p_k\}$ are all known and given at sampling.

% \end{enumerate}

% \item Add all the other join-related results we had 

% \end{enumerate}


